Nonlinear dynamics of localization in neural receptive fields

Localized receptive fields -- neurons that are selective for certain contiguous spatiotemporal features of their input -- populate early sensory regions of the mammalian brain. Unsupervised learning algorithms that optimize explicit sparsity or independence criteria replicate features of these localized receptive fields, but fail to explain directly how localization arises through learning without efficient coding, as occurs in early layers of deep neural networks and might occur in early sensory regions of biological systems. We consider an alternative model in which localized receptive fields emerge without explicit top-down efficiency constraints -- a feedforward neural network trained on a data model inspired by the structure of natural images. Previous work identified the importance of non-Gaussian statistics to localization in this setting but left open questions about the mechanisms driving dynamical emergence. We address these questions by deriving the effective learning dynamics for a single nonlinear neuron, making precise how higher-order statistical properties of the input data drive emergent localization, and we demonstrate that the predictions of these effective dynamics extend to the many-neuron setting. Our analysis provides an alternative explanation for the ubiquity of localization as resulting from the nonlinear dynamics of learning in neural circuits.

==> figures/experiments/fig.tex <==
\begin{figure}[t]
  \centering
 \begin{subfigure}{0.95\textwidth}
    \begin{tabular}{ccccc}
      \includegraphics[width=0.25\linewidth]{figures/theory/rf_sim/ising_varphi.pdf} &
      \includegraphics[width=0.25\linewidth]{figures/theory/rf_sim/ising_varphi.pdf} \\ 
      \includegraphics[width=0.25\linewidth]{figures/theory/rf_sim/gaussian_varphi.pdf} &
      \includegraphics[width=0.25\linewidth]{figures/theory/rf_sim/gaussian_varphi.pdf} \\ 
      \includegraphics[width=0.25\linewidth]{figures/theory/rf_sim/alg5_varphi.pdf} &
      \includegraphics[width=0.25\linewidth]{figures/theory/rf_sim/alg5_varphi.pdf} \\ 
    \end{tabular}
  \end{subfigure}
  \caption{
    \nbr{Current figures are placeholders, from Fig. 3.}
    (\textbf{Left})
    \nb{Figure comparing empirical and analytical/approximated receptive fields}
    (\textbf{Right})
    \nb{Figure showing ICA components in 1D, 2D cases}
  }
  \label{fig:experiments}
\end{figure}


==> figures/peak-failure/fig.tex <==
\begin{wrapfigure}{l}{0.95\textwidth}
  \vspace{-6pt}
  \scalebox{0.9}{
    \hspace{-8pt}
    \begin{tabular}{m{1pt}cc}
      \raisebox{110pt}{
      \rotatebox{90}{magnitude $w_i$}
      }
      &
      \hspace{8pt}\includegraphics[width=0.5\linewidth]{figures/peak-failure/ising.pdf}
      &
      \includegraphics[width=0.5\linewidth]{figures/peak-failure/ising_kurtosis.pdf}  \\
      \noalign{\vskip -84pt}
      & 
      \hspace{22pt}
      dimension $i$ of weight $\mathbf{w}$ & 
      \hspace{22pt}
      dimension $i$ of weight $\mathbf{w}$ 
    \end{tabular}
  }
  \caption{
    Failure case for peak prediction, as discussed in \cref{sec:peak-prediction}.
    The (\textbf{left}) simulated receptive field localizes with a peak at index $i=21$, while the (\textbf{right}) integrated receptive field localizes at $i=3$.
    This is because localization is extremely sensitive to initial conditions in the weights $\mathbf{w}$.
    This sensitivity manifests as a second bump near $i=3$ for the simulated receptive field earlier in training (darker lines).
    In the integrated receptive field, there is a large bump near $i=21$ early in training, which corresponds to the true peak location.
    Thus, our approximation in integrating identifies these competing bumps, but predicts the wrong one wins out.
  }
  \label{fig:peak-failure}
\end{wrapfigure}


==> paratext/neurips-checklist.tex <==
\section*{NeurIPS Paper Checklist}
\begin{enumerate}
\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, in the abstract and introduction we claim to derive an 
      analytical model for the effective dynamics of localization (\cref{sec:theory}) 
      in the setting described in \cref{sec:prelims}
      and validate this model with experiments (\cref{sec:experiments}).
\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, in the conclusion we note that our exact analysis is retricted to 
      the single-neuron architecture \labelcref{item:single-neuron-model} in the data setting described in \cref{sec:prelims},
      and that validations beyond that scope (like in \cref{sec:experiments}) remain empirical even if they show promise.
\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, our assumptions are rigourously stated in \cref{sec:theory} and the proofs are provided in \cref{app:proofs}.
\item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Our setup (\cref{sec:experiments}) and experiments (\cref{sec:experiments}) provides full details on the 
      data, hyperparameters, and training procedures used to obtain the figures. We also provide code (referenced on the first page).
\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, we provide a link to the code repository in the first page of the paper, and the repository contains all the code and data needed to reproduce the experiments.
\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, we provide primary details in \cref{sec:experiments} and all the details in the code.
\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes
    \item[] Justification: Yes, for our prediction experiment in \cref{sec:peak-prediction} we report a measure of variation over multiple runs.
      
\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes
    \item[] Justification: Yes, we provide this information at the beginning of \cref{sec:experiments}.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes
    \item[] Justification: Yes, we have reviewed the NeurIPS Code of Ethics and believe that our work conforms to it.
\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA
    \item[] Justification: Since our work is primarily theoretical analysis of an existing phenomenon, we do not consider it to have 
      direct societal impacts. 
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA
    \item[] Justification: Our work does not involve the release of data or models that have a significant risk for misuse.
\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes
    \item[] Justification: We wrote our own code for all experiments to procedurally generate data and train and analyze models.
      Visualizations from prior work in \cref{fig:sim-real-gabors} are properly credited.
\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes
    \item[] Justification: We document our code (the only asset we release) in the accompanying repository.
\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA
    \item[] Justification: Our paper does not involve crowdsourcing nor research with human subjects.
\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA
    \item[] Justification: Our paper does not involve crowdsourcing nor research with human subjects.
\end{enumerate}

